For the Metatheory of Type Theory, Internal Sconing Is Enough

Metatheorems about type theories are often proven by interpreting the syntax into models constructed using categorical gluing. We propose to use only sconing (gluing along a global section functor) instead of general gluing. The sconing is performed internally to a presheaf category, and we recover the original glued model by externalization. Our method relies on constructions involving two notions of models: first-order models (with explicit contexts) and higher-order models (without explicit contexts). Sconing turns a displayed higher-order model into a displayed first-order model. Using these, we derive specialized induction principles for the syntax of type theory. The input of such an induction principle is a boilerplate-free description of its motives and methods, not mentioning contexts. The output is a section with computation rules specified in the same internal language. We illustrate our framework by proofs of canonicity, normalization and syntactic parametricity for type theory.

==> macros.tex <==
%%% General macros

% Abbreviations.
\makeatletter
\newcommand{\DeclareAbbrevation}[2]{\newcommand{#1}{\@ifnextchar{.}{#2}{#2.\@\xspace}}}
\makeatother

\DeclareAbbrevation{\ie}{i.e}
\DeclareAbbrevation{\eg}{e.g}
\DeclareAbbrevation{\cf}{cf}
\DeclareAbbrevation{\resp}{resp}
\DeclareAbbrevation{\etal}{et al}
\DeclareAbbrevation{\ibid}{ibid}
\DeclareAbbrevation{\ca}{ca}
\DeclareAbbrevation{\vs}{vs}
\DeclareAbbrevation{\etc}{etc}

% End of definitions
\DeclareRobustCommand{\lipicsEnd}{%
  \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \quad\hbox{$\lrcorner$}%
}

% Lowercase mathcal
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}%
{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathcal}{U}{mathc}{m}{it}

% Japanese letters (for the Yoneda embedding)
\DeclareFontFamily{U}{min}{}
\DeclareFontShape{U}{min}{m}{n}{<-> udmj30}{}

% Emphasis
\newcommand{\defemph}[1]{\textbf{#1}}
\newcommand{\deemph}[1]{\textcolor{gray}{#1}}

% Double langle/rangle
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother

% Arrows
\newcommand{\uda}{\updownarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\rat}{\rightarrowtail}
\newcommand{\ratri}{\rightarrowtriangle}
\newcommand{\thra}{\twoheadrightarrow}
\newcommand{\thla}{\twoheadleftarrow}
\newcommand{\rsqa}{\rightsquigarrow}

% Brackets

\newcommand*{\llbrace}{%
  \BeginAccSupp{method=hex,unicode,ActualText=2983}%
    \textnormal{\usefont{OMS}{lmr}{m}{n}\char102}%
    \mathchoice{\mkern-4.05mu}{\mkern-4.05mu}{\mkern-4.3mu}{\mkern-4.8mu}%
    \textnormal{\usefont{OMS}{lmr}{m}{n}\char106}%
  \EndAccSupp{}%
}
\newcommand*{\rrbrace}{%
  \BeginAccSupp{method=hex,unicode,ActualText=2984}%
    \textnormal{\usefont{OMS}{lmr}{m}{n}\char106}%
    \mathchoice{\mkern-4.05mu}{\mkern-4.05mu}{\mkern-4.3mu}{\mkern-4.8mu}%
    \textnormal{\usefont{OMS}{lmr}{m}{n}\char103}%
  \EndAccSupp{}%
}

\newcommand{\parens}[1]{{\left( #1 \right)}}
\newcommand{\abs}[1]{{\left| #1 \right|}}
\newcommand{\sem}[1]{{\llbracket #1 \rrbracket}}
\newcommand{\osem}[1]{{\llbrace #1 \rrbrace}}
\newcommand{\lens}[1]{{\llparenthesis #1 \rrparenthesis}}
\newcommand{\trunc}[1]{{\parallel #1 \parallel}}
\newcommand{\angles}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\uquote}[1]{{\lceil #1 \rceil}}
\newcommand{\dquote}[1]{{\lfloor #1 \rfloor}}

%%% Short names

% Short names for models (mathbb)
\newcommand{\MA}{\mathbb{A}}
\newcommand{\MB}{\mathbb{B}}
\newcommand{\MC}{\mathbb{C}}
\newcommand{\MD}{\mathbb{D}}
\newcommand{\ME}{\mathbb{E}}
\newcommand{\MF}{\mathbb{F}}
\newcommand{\MG}{\mathbb{G}}
\newcommand{\MH}{\mathbb{H}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MJ}{\mathbb{J}}
\newcommand{\MK}{\mathbb{K}}
\newcommand{\ML}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\MN}{\mathbb{N}}
\newcommand{\MO}{\mathbb{O}}
\newcommand{\MP}{\mathbb{P}}
\newcommand{\MQ}{\mathbb{Q}}
\newcommand{\MR}{\mathbb{R}}
\newcommand{\MS}{\mathbb{S}}
\newcommand{\MT}{\mathbb{T}}
\newcommand{\MU}{\mathbb{U}}
\newcommand{\MV}{\mathbb{V}}
\newcommand{\MW}{\mathbb{W}}
\newcommand{\MX}{\mathbb{X}}
\newcommand{\MY}{\mathbb{Y}}
\newcommand{\MZ}{\mathbb{Z}}


\newcommand{\Ma}{\mathbb{a}}
\newcommand{\Mb}{\mathbb{b}}
\newcommand{\Mc}{\mathbb{c}}
\newcommand{\Md}{\mathbb{d}}
\newcommand{\Me}{\mathbb{e}}
\newcommand{\Mf}{\mathbb{f}}
\newcommand{\Mg}{\mathbb{g}}
\newcommand{\Mh}{\mathbb{h}}
\newcommand{\Mi}{\mathbb{i}}
\newcommand{\Mj}{\mathbb{j}}
\newcommand{\Mk}{\mathbb{k}}
\newcommand{\Ml}{\mathbb{l}}
\newcommand{\Mm}{\mathbb{m}}
\newcommand{\Mn}{\mathbb{n}}
\newcommand{\Mo}{\mathbb{o}}
\newcommand{\Mp}{\mathbb{p}}
\newcommand{\Mq}{\mathbb{q}}
\newcommand{\Mr}{\mathbb{r}}
\newcommand{\Ms}{\mathbb{s}}
\newcommand{\Mt}{\mathbb{t}}
\newcommand{\Mu}{\mathbb{u}}
\newcommand{\Mv}{\mathbb{v}}
\newcommand{\Mw}{\mathbb{w}}
\newcommand{\Mx}{\mathbb{x}}
\newcommand{\My}{\mathbb{y}}
\newcommand{\Mz}{\mathbb{z}}


% Short names for sets and internal things (mathrm / mathsf)
\newcommand{\SProp}{\mathrm{Prop}}
\newcommand{\SSet}{\mathrm{Set}}
\newcommand{\SCat}{\mathrm{Cat}}
\newcommand{\SCwf}{\mathrm{CwF}}

\newcommand{\cxl}{\mathsf{cxl}}
\newcommand{\cof}{\mathsf{cof}}
\newcommand{\dem}{\mathsf{dem}}

\newcommand{\SA}{\mathsf{A}}
\newcommand{\SB}{\mathsf{B}}
\newcommand{\SC}{\mathsf{C}}
\newcommand{\SD}{\mathsf{D}}
\newcommand{\SE}{\mathsf{E}}
\newcommand{\SF}{\mathsf{F}}
\newcommand{\SG}{\mathsf{G}}
\newcommand{\SH}{\mathsf{H}}
\newcommand{\SI}{\mathsf{I}}
\newcommand{\SJ}{\mathsf{J}}
\newcommand{\SK}{\mathsf{K}}
\newcommand{\SL}{\mathsf{L}}
\newcommand{\SM}{\mathsf{M}}
\newcommand{\SN}{\mathsf{N}}
\newcommand{\SO}{\mathsf{O}}
\newcommand{\SP}{\mathsf{P}}
\newcommand{\SQ}{\mathsf{Q}}
\newcommand{\SR}{\mathsf{R}}
\renewcommand{\SS}{\mathsf{S}}
\newcommand{\ST}{\mathsf{T}}
\newcommand{\SU}{\mathsf{U}}
\newcommand{\SV}{\mathsf{V}}
\newcommand{\SW}{\mathsf{W}}
\newcommand{\SX}{\mathsf{X}}
\newcommand{\SY}{\mathsf{Y}}
\newcommand{\SZ}{\mathsf{Z}}

\newcommand{\Sa}{\mathsf{a}}
\newcommand{\Sb}{\mathsf{b}}
\newcommand{\Sc}{\mathsf{c}}
\newcommand{\Sd}{\mathsf{d}}
\newcommand{\Se}{\mathsf{e}}
\newcommand{\Sf}{\mathsf{f}}
\newcommand{\Sh}{\mathsf{h}}
\newcommand{\Sg}{\mathsf{g}}
\newcommand{\Si}{\mathsf{i}}
\newcommand{\Sj}{\mathsf{j}}
\newcommand{\Sk}{\mathsf{k}}
\newcommand{\Sl}{\mathsf{l}}
\newcommand{\Sm}{\mathsf{m}}
\newcommand{\Sn}{\mathsf{n}}
\newcommand{\So}{\mathsf{o}}
\newcommand{\Sp}{\mathsf{p}}
\newcommand{\Sq}{\mathsf{q}}
\newcommand{\Sr}{\mathsf{r}}
\newcommand{\Ss}{\mathsf{s}}
\newcommand{\St}{\mathsf{t}}
\newcommand{\Su}{\mathsf{u}}
\newcommand{\Sv}{\mathsf{v}}
\newcommand{\Sw}{\mathsf{w}}
\newcommand{\Sx}{\mathsf{x}}
\newcommand{\Sy}{\mathsf{y}}
\newcommand{\Sz}{\mathsf{z}}

% Short names for categories (mathbf or mathcal)
\newcommand{\CSet}{\mathbf{Set}}
\newcommand{\CProp}{\mathbf{Prop}}
\newcommand{\CPsh}{\mathbf{Psh}}
\newcommand{\CCat}{\mathbf{Cat}}
\newcommand{\CCwf}{\mathbf{CwF}}
\newcommand{\CMod}{\mathbf{Mod}}

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

\newcommand{\BA}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\BC}{\mathbf{C}}
\newcommand{\BD}{\mathbf{D}}
\newcommand{\BE}{\mathbf{E}}
\newcommand{\BF}{\mathbf{F}}
\newcommand{\BG}{\mathbf{G}}
\newcommand{\BH}{\mathbf{H}}
\newcommand{\BI}{\mathbf{I}}
\newcommand{\BJ}{\mathbf{J}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\newcommand{\BM}{\mathbf{M}}
\newcommand{\BN}{\mathbf{N}}
\newcommand{\BO}{\mathbf{O}}
\newcommand{\BP}{\mathbf{P}}
\newcommand{\BQ}{\mathbf{Q}}
\newcommand{\BR}{\mathbf{R}}
\newcommand{\BS}{\mathbf{S}}
\newcommand{\BT}{\mathbf{T}}
\newcommand{\BU}{\mathbf{U}}
\newcommand{\BV}{\mathbf{V}}
\newcommand{\BW}{\mathbf{W}}
\newcommand{\BX}{\mathbf{X}}
\newcommand{\BY}{\mathbf{Y}}
\newcommand{\BZ}{\mathbf{Z}}

% mathfrak letters
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}

%%% Category theory

% Categorical structure
\newcommand{\Ob}{\mathsf{Ob}}
\newcommand{\Hom}{\mathsf{Hom}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\op}{\mathsf{op}}

% Colimits
\DeclareMathOperator*{\colim}{colim}

% Presheaf categories
\newcommand{\psh}[1]{\widehat{#1}}
\newcommand{\yo}{\text{\usefont{U}{min}{m}{n}\symbol{'210}}}
% \newcommand{\yo}{\mathbbm{y}}

\newcommand{\rep}{\mathsf{rep}}
\newcommand{\UPsh}{\UU}
\newcommand{\URepPsh}{\UU_{\rep}}

%%% Type theory

% Components of models of type theory
\newcommand{\type}{\mathsf{type}}
\newcommand{\Con}{\mathsf{Con}}
\newcommand{\Sub}{\mathsf{Sub}}
\newcommand{\Ty}{\mathsf{Ty}}
\newcommand{\ty}{\mathsf{ty}}
\newcommand{\Tm}{\mathsf{Tm}}
\newcommand{\tm}{\mathsf{tm}}
\newcommand{\Var}{\mathsf{Var}}
\newcommand{\var}{\mathsf{var}}

% Booleans
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\BoolTy}{\mathsf{Bool}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\elimBool}{\mathsf{elim}_{\BoolTy}}

% Natural numbers
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\NatTy}{\mathbf{N}}
\newcommand{\zero}{\mathsf{zero}}
\newcommand{\suc}{\mathsf{suc}}
\newcommand{\elimNat}{\mathsf{elim}_{\NatTy}}

% Id-types
\newcommand{\Id}{\mathsf{Id}}
\newcommand{\J}{\mathsf{J}}
\newcommand{\Jbeta}{{\mathsf{J}\beta}}
\newcommand{\refl}{\mathsf{refl}}
\newcommand{\ap}{\mathsf{ap}}
\newcommand{\tr}{\mathsf{tr}}
\newcommand{\happly}{\mathsf{happly}}

% Eq-types
\newcommand{\Eq}{\mathsf{Eq}}

% Equivalences / hLevels
\newcommand{\Equiv}{\mathrm{Equiv}}
\newcommand{\isEquiv}{\mathrm{isEquiv}}
\newcommand{\isContr}{\mathrm{isContr}}
\newcommand{\isProp}{\mathrm{isProp}}
\newcommand{\isSet}{\mathrm{isSet}}
\newcommand{\isLinv}{\mathrm{isLInv}}
\newcommand{\isRinv}{\mathrm{isRInv}}

% Pi-types
\newcommand{\app}{\mathsf{app}}
\newcommand{\lam}{\mathsf{lam}}
\newcommand{\funext}{\mathsf{funext}}

% Sigma and Unit-types
\newcommand{\pair}{\mathsf{pair}}
\newcommand{\fst}{\mathsf{fst}}
\newcommand{\snd}{\mathsf{snd}}

\newcommand{\Unit}{\mathbf{1}}
\renewcommand{\tt}{\mathsf{tt}}

\newcommand{\Init}{\mathbf{0}}
\newcommand{\absurd}{\mathsf{absurd}}

% Quotients
\newcommand{\Quot}{\mathbf{Q}}
\newcommand{\quot}{\mathbf{q}}

% Universes
\newcommand{\UU}{\mathcal{U}}
\newcommand{\UV}{\mathcal{V}}

% Circled dollar symbol
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.1pt] (char) {#1};}}
\newcommand{\circleddollar}{\mathbin{\circled{\scalebox{0.7}{$\$$}}}}

% MTT Colors
\newcommand{\modcolor}[1]{\textcolor{orange!60!black}{#1}}
\newcommand{\natcolor}[1]{\textcolor{teal}{#1}}
\newcommand{\tickcolor}[1]{\textcolor{white!70!black}{#1}}

% Multimodal type theory

\newcommand{\modm}[1]{\{\modcolor{#1}\}} % Modality
\newcommand{\modt}[1]{\{\tickcolor{#1}\}} % Tick
\newcommand{\modtm}[2]{\{\tickcolor{#1} \colon\modcolor{#2}\}} % Tick and modality

\newcommand{\keyn}[1]{[\natcolor{#1}]} % (natural) transformation
\newcommand{\keytt}[2]{[\tickcolor{#1} / \tickcolor{#2}]} % tick -> tick
\newcommand{\keymm}[2]{[\modcolor{#1} / \modcolor{#2}]} % mod -> mod
\newcommand{\keyntt}[3]{[\natcolor{#1} \colon\tickcolor{#2} / \tickcolor{#3}]} % natural transformation : tick -> tick
\newcommand{\keynmm}[3]{[\natcolor{#1} \colon\modcolor{#2} / \modcolor{#3}]} % natural transformation : mod -> mod

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

